DiffSal: Joint Audio and Video Learning for Diffusion Saliency Prediction

Audio-visual saliency prediction can draw support from diverse modality complements, but further performance enhancement is still challenged by customized architectures as well as task-specific loss functions. In recent studies, denoising diffusion models have shown more promising in unifying task frameworks owing to their inherent ability of generalization. Following this motivation, a novel Diffusion architecture for generalized audio-visual Saliency prediction (DiffSal) is proposed in this work, which formulates the prediction problem as a conditional generative task of the saliency map by utilizing input audio and video as the conditions. Based on the spatio-temporal audio-visual features, an extra network Saliency-UNet is designed to perform multi-modal attention modulation for progressive refinement of the ground-truth saliency map from the noisy map. Extensive experiments demonstrate that the proposed DiffSal can achieve excellent performance across six challenging audio-visual benchmarks, with an average relative improvement of 6.3\% over the previous state-of-the-art results by six metrics.

==> sec/sec_abstract.tex <==
\begin{abstract}
Audio and video signals can be used jointly for saliency prediction as they complement each other. However, most audio-visual saliency prediction methods resort to using customized architectures as well as task-specific loss functions. In this work, we present a novel  \textbf{Diff}usion architecture for generalized audio-visual \textbf{Sal}iency prediction (DiffSal), which formulates the prediction problem as a conditional generative task of the saliency map via utilizing input video and audio as the condition.
In addition to extracting spatio-temporal video and audio features from image sequences and corresponding audio signals, a Saliency-UNet is designed to perform multi-modal attention modulation to progressively refine the ground-truth saliency map from the noisy map.
Extensive experiments demonstrate that the proposed DiffSal achieves excellent performance across six challenging audio-visual benchmarks, with an average relative improvement of 6.3\% over the previous state-of-the-art results in six metrics.

%In this work, we present DiffSal, a novel conditional diffusion saliency model with the benefits of generalized network structure and effective audio-visual interaction.

%The prediction problem is formulated  as a conditional generative task of saliency map, utilizing input video and audio features as condition.




%The saliency predictions are iteratively generated from random noise with input video and audio features as condition.

%Extensive experiments demonstrate that the proposed \textbf{DiffSal} achieves superior performance across seven challenging  benchmarks for two tasks, and significantly outperforms the other state-of-the-art methods. 

%While many approaches have crafted task-specific training paradigms for either video saliency prediction or video salient object detection tasks, few attention has been devoted to devising a generalized saliency modeling framework that seamlessly bridges both these distinct tasks.

%introduce the \textbf{Uni}fied \textbf{S}aliency \textbf{T}ransformer (\textbf{UniST}) framework, which  comprehensively utilizes the essential attributes of video saliency prediction and video salient object detection. 

%learn the spatio-temporal representations at progressively  increased resolutions, while incorporating effective cross-scale  saliency information to produce a robust representation.  


%Furthermore, a task-specific decoder is proposed to perform the final prediction for each task.

%To the best of our knowledge, this is the first work that explores designing a transformer structure for both saliency modeling tasks. 



%Video saliency prediction and detection are thriving research domains that enable computers to simulate the distribution of visual attention akin to how humans perceiving dynamic scenes.

\end{abstract}

==> sec/sec_experiment_new.tex <==
\section{Experiments}
The implementation details and evaluation metrics are presented in the following subsections. Experiments are conducted on six audio-visual datasets and the results are reported with analysis of ablation studies and comparison of state-of-the-art works.

\subsection{Setup}
\noindent \textbf{Audio-Visual Datasets}: Six audio-visual datasets in saliency prediction have been employed for the evaluation, which are: AVAD \cite{min2016fixation}, Coutrot1 \cite{coutrot2014saliency}, Coutrot2 \cite{coutrot2016multimodal}, DIEM \cite{mital2011clustering}, ETMD \cite{koutras2015perceptually}, and SumMe \cite{gygli2014creating}. The significant characteristics of these datasets are elaborated as below.
(i) The AVAD dataset comprises 45 video clips with durations ranging from 5 to 10 seconds. These clips cover various audio-visual activities, such as playing the piano, playing basketball, conducting interviews, \etc. This dataset contains eye-tracking data from 16 participants.
(ii) The Coutrot1 and Coutrot2 datasets are derived from the Coutrot dataset. Coutrot1 consists of 60 video clips covering four visual categories: one moving object, several moving objects, landscapes, and faces. The corresponding eye-tracking data are obtained from 72 participants. Coutrot2 includes 15 video clips recording four individuals having a meeting, with eye-tracking data from 40 participants.
(iii) The DIEM dataset contains 84 video clips, including game trailers, music videos, advertisements, \etc., captured from 42 participants. Notably, the audio and visual tracks in these videos do not naturally correspond.
(iv) The ETMD dataset comprises 12 video clips extracted from various Hollywood movies, with eye-tracking data annotated by 10 different persons.
(v) The SumMe dataset consists of 25 video clips covering diverse topics, such as playing ball, cooking, traveling, \etc.
%The corresponding eye-tracking data are collected from 10 viewers.


\begin{table}[t]
	\centering
	\renewcommand\arraystretch{1.2}
	\caption{Ablation of different components in DiffSal.}
	\vspace{-5pt}
	\resizebox{0.85 \linewidth}{!}{
		\begin{tabular}{l ll llll}
			\toprule
			%			\multirow{2}{*}{Method} & \multirow{2}{*}{ECAM} & \multirow{2}{*}{MIM} & \multicolumn{2}{c}{\textbf{AVAD}}  & \multicolumn{2}{c}{\textbf{\textrm{ETMD}}}  \\
			\multirow{2}{*}{Method} & \multicolumn{2}{c}{Components} & \multicolumn{2}{c}{\textbf{AVAD}}  & \multicolumn{2}{c}{\textbf{\textrm{ETMD}}} \\
			\cmidrule(r){2-3} \cmidrule(r){4-5}  \cmidrule(r){6-7}
			& 			ECA& 		MIM& 	CC $\uparrow$    & SIM $\uparrow$ & CC $\uparrow$   & SIM $\uparrow$  \\
			\midrule
			baseline      &             	&      			 & 0.701 		 & 0.547          & 0.632           & 0.498     \\
			& \checkmark  &         	    & 0.716			 & 0.556          & 0.644           & 0.503    \\
			&   		 &   \checkmark 	& 0.714			 & 0.551          & 0.638           & 0.502   \\
			& \checkmark &  \checkmark   	& \textbf{0.738} & \textbf{0.571} & \textbf{0.652}  & \textbf{0.506}    \\
			\bottomrule
	\end{tabular}}
	\vspace{-15pt}
	\label{table-ablation_1}
\end{table}

%To facilitate implementation, we use pre-trained  MViTv2  model \cite{li2022mvitv2} on Kinetics \cite{carreira2017quo} and pre-trained VGGish \cite{hershey2017cnn} on AudioSet \cite{gemmeke2017audio}.

\noindent \textbf{Implementation Details}: To facilitate implementation, a pre-trained MViTv2 \cite{li2022mvitv2} model on Kinetics \cite{carreira2017quo} and a pre-trained VGGish \cite{hershey2017cnn} on AudioSet \cite{gemmeke2017audio} are adopted. The input samples of the network consist of 16-frame video clips of size $224 \times 384 \times 3$ with the corresponding audio, which is transformed into $9$ slices  of $112 \times 192$ log-Mel spectrograms. For the spatio-temporal compression in efficient spatio-temporal cross-attention, the kernel size and stride size of the 3D convolution in the $i$th MAM stage are set to $2^i$ and $2^i$, respectively. For a fair comparison, the video branch of DiffSal is pre-trained using the DHF1k dataset \cite{wang2018revisiting} following \cite{xiong2023casp}, and the entire model is fine-tuned on these audio-visual datasets using this pre-trained weight.

The training process chooses Adam as the optimizer with the started learning rate of 1e-4. The computation platform is configured by four NVIDIA GeForce RTX 4090 GPUs in a distributed fashion, using Pytorch. The total sampling step $T$ is defined as $1000$ and the entire training is terminated within 5 epochs. The batch size is set to 20 across all experiments. During inference, the iterative denoising step is set to 4.


\noindent \textbf{Evaluation Metrics}: Four widely-accepted evaluation metrics are used \cite{bylinskii2018different}: CC, NSS, AUC-Judd (AUC-J), and SIM, which is the same as being used in previous works \cite{tsiami2020stavis,xiong2023casp}.



\subsection{Ablation Studies}
Extensive ablation studies are performed to validate the design choices for different functional modules. The AVAD and ETMD datasets are selected for ablation studies, following the approach in \cite{xiong2023casp}.

\begin{table}[t]
	\centering
	\renewcommand\arraystretch{1.2}
	\caption{Ablation of video and audio modalities.}
	\vspace{-5pt}
	\resizebox{0.7 \linewidth}{!}{
		\begin{tabular}{l llll}
			\toprule
			\multirow{2}{*}{Model} &  \multicolumn{2}{c}{\textbf{AVAD}}  & \multicolumn{2}{c}{\textbf{\textrm{ETMD}}}  \\
			\cmidrule(r){2-3} \cmidrule(r){4-5}
			&  CC $\uparrow$ & SIM $\uparrow$ & CC $\uparrow$ & SIM $\uparrow$   \\
			\midrule
			Audio-Only       & 0.343 & 0.283 & 0.362  & 0.295  \\
			Video-Only       & 0.716 & 0.556  & 0.644  & 0.503  \\
			Ours             & \textbf{0.738} & \textbf{0.571} & \textbf{0.652} & \textbf{0.506} \\
			\bottomrule
	\end{tabular}}
	\label{table-ablation_av_encoders}
	\vspace{-10pt}
\end{table}

\begin{figure}[t]
	%	\flushleft
	\centering
	\includegraphics[scale=0.5]{figures/fig_audio_maps.pdf}
	\vspace{-10pt}
	\caption{Visualizing the saliency results when different modalities are used. The audio-only approach is able to localize the sound source coming from the performer's guitar, while the video-only approach focuses on both the performer's face as well as  the guitar.}
	\vspace{-15pt}
	\label{fig-ablation-av-encoders}
\end{figure}

\noindent \textbf{Effect of Components of DiffSal}.
%In the experimental Table \ref{table-ablation_1}, the aim is to investigate the effectiveness of each proposed component. A strong baseline method is first employed which models the video-only version of DiffSal framework, replacing the designed multi-modal attention modulation with the purely convolution operation.


To validate the effectiveness of each module in proposed framework, a baseline model is initially defined as the video-only version of DiffSal, and replaces the multi-modal attention modulation in Saliency-UNet with a pure convolution operation.

As shown in Table \ref{table-ablation_1}, the baseline model demonstrates a good performance that indicates a potential capability of diffusion-based framework in AVSP task. With incorporation of the designed efficient spatio-temporal cross-attention (ECA), and the multi-modal interaction module (MIM) components, the overall performance of the model has been enhanced continually. As the core module, ECA presents a significant improvement in the CC metric by 0.015 on the AVAD dataset, and 0.012 on the ETMD dataset for the whole DiffSal framework. With the addition of the audio features and the MIM, the model also has another improvement of 0.013 in the CC metric on the AVAD dataset. All of these have demonstrated an effectiveness of ECA and MIM in the proposed DiffSal.


%We perform ablation experiments to investigate the effectiveness of each proposed component, and report the results in Table \ref{table-ablation_1}. We first define a strong baseline method representing the audio-visual saliency model using the original DiffSal framework. The model is a purely visual version of DiffSal framework, while replacing the multi-modal attention modulation structure devised in this paper with a purely convolutional operation. From Table \ref{table-ablation_1}, the baseline model demonstrates good performance, suggesting that the diffusion-based approach has strong potential for the AVSP task. The performance of the model is continuously improved by adding the designed efficient cross-attention mechanism (ECAM) and multi-modal interaction module (MIM) components to the baseline method. Specifically, as the core module of the DiffSal framework, ECAM significantly improves the CC metric by 0.018 on the AVAD dataset, and 0.015 on the ETMD dataset. With the addition of the audio features and the MIM, the model also has an improvement of 0.021 in the CC metric on the AVAD dataset.


%\begin{table}[t]
%	\centering
%	\renewcommand\arraystretch{1.2}
%	\caption{Ablation of Video and Audio Modalities.}
%	\resizebox{0.9 \linewidth}{!}{
	%		\begin{tabular}{l llll ll}
		%			\toprule
		%			\multirow{2}{*}{Model} &  \multicolumn{2}{c}{\textbf{AVAD}}  & \multicolumn{2}{c}{\textbf{\textrm{DHF1K}}} & \multirow{2}{*}{\#Params} & \multirow{2}{*}{\#FLOPs} \\
		%			\cmidrule(r){2-3} \cmidrule(r){4-5}
		%			&  CC $\uparrow$ & SIM $\uparrow$ & CC $\uparrow$ & SIM $\uparrow$   \\
		%			\midrule
		%			Our(w/ Audio)      				 		& 0.343 & 0.283 & -  & - & \textbf{45.75M} &  \textbf{106.27G} \\
		%			CASP-Net\cite{xiong2023casp} 			& 0.691 & 0.528 &- &-  &  51.62M & 283.35G  \\
		%
		%			\midrule
		%			Our(w/ Video)      						 & 0.719 & 0.556  & 0.533  & 0.405 & 73.82M & 165.21G \\
		%			TMFI-Net \cite{zhou2023transformer}	  	& - & - & 0.524 &0.410  & 53.41M & 305.15G \\
		%			\midrule
		%			Ours             						& \textbf{0.737} & \textbf{0.571} & \textbf{0.652}  & \textbf{0.509} & 79.85M & 191.45G \\
		%			\bottomrule
		%			
		%	\end{tabular}}
%	\label{table-ablation_av_encoders2}
%\end{table}


\noindent \textbf{Effect of Video and Audio Modalities}.
Table \ref{table-ablation_av_encoders} shows the contribution of spatio-temporal information from each modality in the Video and Audio Encoders to the overall performance. The experimental results reveal that video-only model exhibit significantly greater strength than spatio-temporal audio-only, which verifies the essential role of the video modality. Figure \ref{fig-ablation-av-encoders} also visualizes the model predictions using two modal encoders separately. It is clear that either the audio-only or video-only approach can predict saliency areas in the scene, and the combination of the two modalities leads to more accurate predictions. This demonstrates the generalization of the DiffSal framework to audio-only, video-only, and audio-visual scenarios as well.

%This showcases the generalizability  of our DiffSal framework, which proves effective not only in AVSP tasks in multi-modal scenarios but also in uni-modal scenarios where a certain modality is absent.
%Considering that both video and audio features encode spatio-temporal information, we further investigate the contribution of the spatio-temporal information of each modality in the  Video and Audio Encoders to the overall performance in Table \ref{table-ablation_av_encoders}. We observe that the video features alone are much stronger than the spatio-temporal audio features, and that video plays an important role. We also visualize the results for the approach that uses two modal encoders separately. In Figure \ref{fig-ablation-av-encoders}, it can be seen that our method can roughly predict the saliency areas in the scene using only the audio modality, and even sometimes agrees with the predictions of the video-only method. This reflects the fact that our DiffSal framework is not only applicable to AVSP tasks in multi-modal scenarios but also to uni-modal scenarios where a certain modality is missing.

\begin{table}[t]
	\centering
	\renewcommand\arraystretch{1.2}
	\caption{Ablation of different multi-modal interaction methods.}
	\vspace{-5pt}
	\resizebox{0.8 \linewidth}{!}{
		\begin{tabular}{l llll}
			\toprule
			%			\multirow{2}{*}{Method} & \multirow{2}{*}{ECAM} & \multirow{2}{*}{MIM} & \multicolumn{2}{c}{\textbf{AVAD}}  & \multicolumn{2}{c}{\textbf{\textrm{ETMD}}}  \\
			\multirow{2}{*}{Method}  & \multicolumn{2}{c}{\textbf{AVAD}}  & \multicolumn{2}{c}{\textbf{\textrm{ETMD}}} \\
			\cmidrule(r){2-3} \cmidrule(r){4-5}
			& 		 	CC $\uparrow$    & SIM $\uparrow$ & CC $\uparrow$   & SIM $\uparrow$  \\
			\midrule
			DiffSal(w/ MIM)						& \textbf{0.738} & \textbf{0.571} & \textbf{0.652}  & \textbf{0.506}    \\
			\midrule
			\quad w/ Bilinear						& 0.716			 & 0.556          & 0.644           & 0.503    \\
			\quad w/ Addition						& 0.706			 & 0.543          & 0.606           & 0.464     \\
			\quad w/ Concatenation				& 0.716			 & 0.556          & 0.644           & 0.503   \\
			\bottomrule
	\end{tabular}}
	\label{table-ablation-fusion}
	\vspace{-5pt}
\end{table}




\begin{table}[t]
	\centering
	\renewcommand\arraystretch{1.2}
	\caption{Ablation of different cross-attention strategies. The computational cost is evaluated based on input audio of size $1 \times 9 \times 112 \times 192$ and video of size  $3 \times 16 \times 224 \times 384$. \# Params and \#Mem denote the number of parameters and memory footprint of the model, respectively.}
		\vspace{-5pt}
	\resizebox{0.9 \linewidth}{!}{
			\begin{tabular}{l llll ll}
					\toprule
					\multirow{2}{*}{Attention}  & \multirow{2}{*}{\#Params} & \multirow{2}{*}{\#Mem} &  \multicolumn{2}{c}{\textbf{AVAD}}  & \multicolumn{2}{c}{\textbf{\textrm{ETMD}}}  \\
					\cmidrule(r){4-5} \cmidrule(r){6-7}
					& & &  CC $\uparrow$ & SIM $\uparrow$ & CC $\uparrow$ & SIM $\uparrow$   \\
					\midrule
					SCA 	  & 76.43M & 5.32G	& 0.713 & 0.531 & 0.628 & 0.476    \\
					ECA 	  &  76.57M & 1.20G		& \textbf{0.737} & \textbf{0.571} & \textbf{0.652}  & \textbf{0.509}  \\     				
					\bottomrule
					
			\end{tabular}}
		\vspace{-10pt}
	\label{table-ablation_CA}
\end{table}

\noindent \textbf{Effect of Different Cross-Attention Strategies}. The design of efficient spatio-temporal cross-attention mechanism is further evaluated. As shown in Table \ref{table-ablation_CA}, using efficient spatio-temporal cross-attention (ECA) not only leads to better performance, but also greatly reduces the memory footprint of the model compared to using the standard cross-attention (SCA) strategy. This shows that the designed ECA is able to compress the effective spatio-temporal cues in the features, and reduce the interference of irrelevant noises.

\noindent \textbf{Effect of Different Multi-modal Interaction Methods}. The effects of using different multi-modal interaction methods, such as Bilinear \cite{tenenbaum2000separating}, Addition, and Concatenation, are compared in Table \ref{table-ablation-fusion}. These multi-modal interaction can be found in recent state-of-the-art works \cite{tsiami2020stavis, jain2021vinet}, and the video features and noise features are firstly concatenated before their interaction with audio features. Experimental results show that the proposed MIM is able to outperform all the other three interaction methods, and obtain more robust multi-modal features. In contrast, the performance degradation of the other three methods suffer from the noise information embedded in the features.


\begin{table}[t]
	\centering
	\renewcommand\arraystretch{1.2}
	\caption{Ablation of different training losses.}
	\vspace{-5pt}
	\resizebox{0.9 \linewidth}{!}{
		\begin{tabular}{l lll llll}
			\toprule
			\multirow{2}{*}{Model}  &  \multicolumn{3}{c}{Losses}  & \multicolumn{2}{c}{\textbf{AVAD}}  & \multicolumn{2}{c}{\textbf{\textrm{ETMD}}}  \\
			\cmidrule(r){2-4} \cmidrule(r){5-6}  \cmidrule(r){7-8}
			& $\mathcal{L}_{CE}$& $\mathcal{L}_{KL}$& $\mathcal{L}_{MSE}$& CC $\uparrow$  & SIM $\uparrow$ & CC $\uparrow$ & SIM $\uparrow$  \\
			\midrule
			
			\multirow{3}{*}{Ours} & $\checkmark$ & & & 0.690 & 0.490 & 0.617  & 0.422     \\
			& & $\checkmark$ & &0.720 & 0.552 & 0.644  & 0.496   \\
			& & & $\checkmark$ & \textbf{0.738} & \textbf{0.571} & \textbf{0.652}  & \textbf{0.506}    \\
			\bottomrule
	\end{tabular}}
	\vspace{-15pt}
	\label{table-ablation_loss}
\end{table}

\begin{figure}[!tbp]
	\hspace{-1cm}
	\flushright
	\begin{minipage}[t]{0.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/fig_denosing_steps_CC.eps}
	\end{minipage}
	\begin{minipage}[t]{0.49\linewidth}
		\centering
		\includegraphics[width=\linewidth]{figures/fig_denosing_steps_SIM.eps}
	\end{minipage}
	\vspace{-10pt}
	\caption{Performance analysis of denoising steps on AVAD and DIEM datasets.}
	\label{fig:exp_denoise_steps}
	\vspace{-10pt}
\end{figure}

\noindent \textbf{Effect of Different Training Losses}. Table \ref{table-ablation_loss} compares the impact on DiffSal using different loss functions from previous state-of-the-art approaches \cite{tsiami2020stavis, xiong2023casp}, such as the cross entropy (CE) loss $\mathcal{L}_{CE}$ and the Kullback-Leibler divergence (KL) loss $\mathcal{L}_{KL}$. During training process, it is observed that the model with the $\mathcal{L}_{CE}$ converges slowly and yields sub-optimal performance. Compared to the $\mathcal{L}_{MSE}$, employing the  $\mathcal{L}_{KL}$ can achieve acceptable results, but there is still a gap with the performance of training with the $\mathcal{L}_{MSE}$. This suggests that simple MSE loss can be used in the AVSP task as an alternative to these task-tailored loss functions.



\begin{table*}[!htbp]
	\begin{center}
		% Table 1.
		\caption{Comparison with state-of-the-art methods on six audio-visual saliency datasets. \textbf{Bold} text in the table indicates the best result, and \underline{underlined} text indicates the second best result. Our DiffSal significantly outperforms the previous state-of-the-arts by a large margin.}
		\label{table-av-sota}
		\vspace*{-5pt}
		\resizebox{0.95\linewidth}{!}{
			\begin{tabular}{c |c|c | cccc | cccc | cccc}
				\toprule
				\multirow{2}*{\textbf{Method}} & \multirow{2}*{\textbf{\#Params}} & \multirow{2}*{\textbf{\#FLOPs}}&  \multicolumn{4}{c|}{\textbf{DIEM}} & \multicolumn{4}{c|}{\textbf{Coutrot1}} & \multicolumn{4}{c}{\textbf{Coutrot2}}\\
				%				\cmidrule(r){2-5}\cmidrule(r){6-9}\cmidrule(r){10-13}%\cline{3-14}
				\cline{4-15}
				& & & CC $\uparrow$ & NSS $\uparrow$ & AUC-J $\uparrow$  & SIM  $\uparrow$&  CC $\uparrow$ & NSS $\uparrow$ & AUC-J$\uparrow$   & SIM $\uparrow$ & CC$\uparrow$ & NSS$\uparrow$ & AUC-J$\uparrow$  & SIM$\uparrow$ \\
				\hline
				$\textrm{ACLNet}_{\mathit{{\rm TPAMI}^\prime} 2019}$  \cite{wang2019revisiting} & - & - & 0.522 & 2.02 & 0.869 & 0.427 & 0.425 & 1.92 & 0.850  & 0.361 & 0.448 & 3.16 & 0.926 &  0.322 \\
				$\textrm{TASED-Net}_{\mathit{{\rm ICCV}^\prime} 2019}$ \cite{min2019tased} & 21.26M & 91.80G & 0.557 & 2.16 & 0.881 & 0.461 & 0.479 & 2.18 & 0.867  & 0.388 & 0.437 & 3.17 & 0.921 &  0.314 \\
				$\textrm{STAViS}_{\mathit{{\rm CVPR}^\prime} 2020}$ \cite{tsiami2020stavis} & 20.76M & 15.31G & 0.579 & 2.26 & 0.883 & 0.482 & 0.472 & 2.11 & 0.868  & 0.393 & 0.734 & 5.28 & 0.958 & 0.511 \\
				$\textrm{ViNet}_{\mathit{\rm IROS}^{\prime} 2021}$ \cite{jain2021vinet} & 33.97M & 115.31G & 0.632 & 2.53 & 0.899  & 0.498 & 0.56 & 2.73 & 0.889  & 0.425 & 0.754 & 5.95 & 0.951 & 0.493 \\
				$\textrm{TSFP-Net}_{\mathit{\rm arXiv}^{\prime} 2021}$ \cite{chang2021temporal} & - & - & 0.651 & \underline{2.62} & 0.906  & 0.527 & \underline{0.571} & \underline{2.73} & \underline{0.895} & 0.447 & 0.743 & 5.31 & 0.959  & 0.528 \\
				$\textrm{CASP-Net}_{\mathit{{\rm CVPR}^\prime} 2023}$ \cite{xiong2023casp} & 51.62M & 283.35G & \underline{0.655} & 2.61 & \underline{0.906}  & \underline{0.543} & 0.561 & 2.65 & 0.889  & \underline{0.456} & \underline{0.788} & \underline{6.34} & \underline{0.963} & \underline{0.585} \\
				%				\midrule
				\hline
				\textbf{Ours}(DiffSal) & 76.57M & 187.31G & \textbf{0.660} & \textbf{2.62} & \textbf{0.907} & \textbf{0.543} & \textbf{0.638} & \textbf{3.20} & \textbf{0.901} & \textbf{0.515} & \textbf{0.835} & \textbf{6.61} & \textbf{0.964} & \textbf{0.625} \\
				%				\bottomrule
				\hline
				\multirow{2}*{\textbf{Method}}  & \multirow{2}*{\textbf{\#Params}} & \multirow{2}*{\textbf{\#FLOPs}} & \multicolumn{4}{c|}{\textbf{AVAD}} & \multicolumn{4}{c|}{\textbf{ETMD}} & \multicolumn{4}{c}{\textbf{SumMe}}\\
				%				\cmidrule(r){2-5}\cmidrule(r){6-9}\cmidrule(r){10-13}
				\cline{4-15}
				& & & CC $\uparrow$ & NSS $\uparrow$ & AUC-J $\uparrow$  & SIM  $\uparrow$&  CC $\uparrow$ & NSS $\uparrow$ & AUC-J$\uparrow$   & SIM $\uparrow$ & CC$\uparrow$ & NSS$\uparrow$ & AUC-J$\uparrow$  & SIM$\uparrow$ \\
				%				\midrule
				\hline
				$\textrm{ACLNet}_{\mathit{{\rm TPAMI}^\prime} 2019}$  \cite{wang2019revisiting} & - & -  & 0.580 & 3.17 & 0.905 & 0.446 & 0.477 & 2.36  & 0.915  & 0.329 & 0.379 & 1.79 & 0.868 &  0.296 \\
				$\textrm{TASED-Net}_{\mathit{{\rm ICCV}^\prime} 2019}$ \cite{min2019tased} & 21.26M & 91.80G& 0.601 & 3.16 & 0.914  & 0.439 & 0.509 & 2.63 & 0.916 & 0.366 & 0.428 & 2.1 & 0.884 & 0.333 \\
				$\textrm{STAViS}_{\mathit{{\rm CVPR}^\prime} 2020}$ \cite{tsiami2020stavis} & 20.76M & 15.31G & 0.608 & 3.18 & 0.919 & 0.457 & 0.569 & 2.94 & 0.931 & 0.425 & 0.422 & 2.04 & 0.888  & 0.337 \\
				$\textrm{ViNet}_{\mathit{\rm IROS}^{\prime} 2020}$ \cite{jain2021vinet} & 33.97M & 115.31G & 0.674 & 3.77 & 0.927 & 0.491 & 0.571 & 3.08 & 0.928 & 0.406 & 0.463 & 2.41 & 0.897  & 0.343 \\
				$\textrm{TSFP-Net}_{\mathit{\rm arXiv}^{\prime} 2021}$  \cite{chang2021temporal} & - & - & \underline{0.704} & 3.77 & 0.932  & 0.521 & 0.576 & 3.07 & 0.932  & 0.428 & 0.464 & 2.30 & 0.894 & 0.360 \\
				$\textrm{CASP-Net}_{\mathit{{\rm CVPR}^\prime} 2023}$ \cite{xiong2023casp} & 51.62M & 283.35G & 0.691 & \underline{3.81} & \underline{0.933} & \underline{0.528} & \underline{0.620} & \underline{3.34} & \underline{0.940} & \underline{0.478} & \underline{0.499} & \underline{2.60} & \underline{0.907} & \underline{0.387} \\
				%				\midrule
				\hline
				\textbf{Ours}(DiffSal) & 76.57M & 187.31G & \textbf{0.737} & \textbf{4.22} & \textbf{0.935} & \textbf{0.571} & \textbf{0.652} & \textbf{3.66} & \textbf{0.943} & \textbf{0.506} & \textbf{0.572} & \textbf{3.14} & \textbf{0.921} & \textbf{0.447} \\
				\bottomrule
		\end{tabular}}
	\end{center}
	\vspace{-5pt}
\end{table*}

\begin{figure*}[!tbp]
	\centering
	\vspace*{-10pt}
	\includegraphics[width=0.95 \textwidth]{figures/fig_visualization_results.pdf}
	\vspace{-10pt}
	\caption{Qualitative results of the proposed work in comparison to the other state-of-the-art works. Challenging scenarios contain fast movement on the tennis court and multiple speakers indoors.
	}
	\label{fig-vis-results}
	\vspace{-10pt}
\end{figure*}

\noindent \textbf{Effect of Denoising Steps}.
The impact of the number of iterative denoising steps on the final performance is studied in Figure \ref{fig:exp_denoise_steps}, it shows that more iteration steps result in better performances. With diminishing marginal benefits as the step number increases, a steady increase in performance is observed. For a linearly increasing of the computational cost with the step number, $N=4$ is used maintains a good balance between performance and computational cost.

%To investigate how the number of iterative steps affects the final performance, we experiment with $N \in_R \{1, \cdots, 12 \} $ and report the results in Figure \ref{fig:exp_denoise_steps}.




\subsection{Method Comparison}
\noindent \textbf{Comparisons with State-of-the-art Methods}. As shown in Table \ref{table-av-sota}, the experimental results of our DiffSal is compared with recent state-of-the-art works on six audio-visual saliency datasets. The table highlights the superiority of DiffSal, as it outperforms the other comparable works on all datasets by defined metrics. Notably, DiffSal significantly surpasses the previous top-performing methods, such as CASP-Net \cite{xiong2023casp} and ViNet \cite{jain2021vinet}, and becomes the new state-of-the-art on these six benchmarks. The performance boost is very encouraging: DiffSal can achieve an average relative performance improvement of up to 6.3\% compared to the second-place performer. Such substantial  improvements validate the effectiveness of the diffusion-based approach as an effective audio-visual saliency prediction framework.


\noindent \textbf{Qualitative Result}. The ability of the model to handle challenging scenarios, such as fast movement on the tennis court and multiple speakers indoors, is further examined. Figure \ref{fig-vis-results} compares the DiffSal against other state-of-the-art approaches, such as CASP-Net \cite{xiong2023casp}, ViNet \cite{jain2021vinet} and STAViS \cite{tsiami2020stavis}. It is observed that DiffSal produces saliency maps much closer to the ground-truth in different challenging scenes. In contrast, CASP-Net mainly focuses on audio-visual consistency and lacks adopting an advanced network structure, leading to sub-optimal results. STAViS is only able to generate the unsurprisingly saliency maps by employing sound source localization.

%CASP-Net is only able to roughly localize to salient regions in the scene due to xxx, making it difficult to focus on salient targets in the regions.


\noindent \textbf{Complexity Analysis}. Table \ref{table-av-sota} illstrates the number of parameters and computational costs of the DiffSal with previous state-of-the-art works. Incorporating Saliency-UNet in DiffSal framework leads to an increase in the number of model parameters compared to CASP-Net. On the other hand, utilizing the efficient cross-attention mechanism decrease the computational complexity of DiffSal to a modest level. From the performance perspective, the DiffSal model can achieve balanced optimal performance with the second-highest computational complexity.


==> sec/sec_intro.tex <==
\section{Introduction}
\label{sec:intro}

Humans can quickly focus on the most interesting areas during their daily activities with the help of their visual and auditory sensory systems. 
The comprehension of visual attention in multi-modal scenarios has been explored by numerous researchers and referred to as an \textit{audio-visual saliency prediction} (AVSP) task.
There are many valuable practical applications for this technology, ranging from video summarization \cite{hu2017deep} and compression \cite{zhu2018spatiotemporal} to virtual reality \cite{7965634} and augmented reality \cite{sitzmann2018saliency}.

%Audio-visual saliency prediction has been extensively studied in computer vision, with the aim of estimating the most prominent area in dynamic audio and video scenes.

%The localization-based and the 3D convolution-based methods use pixel-wise  source localization and multi-scale feature interaction to predict the saliency object, respectively, and both of them methods use confusing combinations of optimization objective.

\begin{figure}
	\centering
	\includegraphics[scale=0.4]{figures/fig_overall.pdf}
	\caption{Comparison of conventional audio-visual saliency prediction paradigms and our proposed diffusion-based approach. 
	Both the localization-based and 3D convolution-based methods use tailored network structures and task-specific loss functions to predict saliency areas.
	Differently, our diffusion-based approach is a generalized audio-visual saliency prediction framework using only the \textit{MSE} objective function.}
	\label{fig-three-methods}
\end{figure}

% and sophisticated loss functions


In recent times, significant efforts have been dedicated to advancing research in this domain, concentrating on elevating the quality of multi-modal interaction and refining the generalizability of model structures.
Among the prevalent AVSP approaches, as depicted in Figure \ref{fig-three-methods}(a), localization-based methods \cite{min2020multimodal, tsiami2020stavis, min2016fixation} have gained attention. These methods typically consider sounding objects in the scene as saliency targets, transforming the saliency prediction task into a spatial sound source localization problem. Although they take into account semantic interactions between audio and visual modalities, their focus on a generalized network structure is limited, resulting in constrained performance.

In contrast, recent 3D convolution-based methods \cite{chang2021temporal, jain2021vinet, yao2021deep, xiong2023casp} exhibit superior performance in predicting audio-visual saliency maps, as illustrated in Figure \ref{fig-three-methods}(b). However, these methods still necessitate customized architectures with built-in inductive bias for the saliency prediction task. For instance, Jain \etal \cite{jain2021vinet} and Xiong \etal \cite{xiong2023casp} both embrace an encoder-decoder structure akin to UNet, but integrate their empirical designs into the decoder. Additionally, Chang \etal \cite{chang2021temporal} employs a complex hierarchical feature pyramid network to aggregate deep semantic features. Moreover, both localization-based and 3D convolution-based methods employ specialized loss functions, contributing to a more intricate audio-visual saliency modeling paradigm.

%Recently, a lot of efforts have been invested in this research area, focusing on enhancing the quality of multimodal interaction as well as improving the generalization of model structure. Among these existing mainstream AVSP approaches, the localization-based methods \cite{min2020multimodal, tsiami2020stavis, min2016fixation}, as shown in Figure \ref{fig-three-methods}(a), typically treat the sounding objects in the scene as saliency targets, which in turn transforms the saliency prediction task into a spatial sound source localization problem, and most of them take full consideration of the semantic interactions between audio and visual modalities. 
%However, they pay little attention to the generalized network structure, leading to low upper limits on the performance of each of these methods. By contrast,  recent  3D convolution-based methods  \cite{chang2021temporal, jain2021vinet, yao2021deep, xiong2023casp} perform better in predicting audio-visual saliency maps, as illustrated in Figure \ref{fig-three-methods}(b). However, such methods still require customized architectures with a built-in inductive bias for the saliency prediction task. For example, Jain \etal \cite{jain2021vinet} and Xiong \etal \cite{xiong2023casp} both adopt an encoder-decoder structure in the style of UNet, but incorporate their empirical designs into the decoder respectively. In addition, Chang \etal \cite{chang2021temporal} employs a complex hierarchical feature pyramid network to aggregate deep semantic features. Moreover, both localization-based and 3D convolution-based methods use tailored loss functions, resulting in a more confusing audio-visual saliency modeling paradigm.


Effective audio-visual interaction and the generalized saliency network are two essential factors for the seamless application of AVSP technology in the real world. Unfortunately, an in-depth exploiting for both challenges in the existing works is far from sufficiency. 
Inspired by the strong generalization ability, diffusion models \cite{ho2020denoising, rombach2022high, ho2022classifier} can be used as a unifying framework for generative tasks, utilizing class labels \cite{dhariwal2021diffusion}, text prompts \cite{gu2022vector}, images  \cite{chen2023diffusiondet}, and even sounds \cite{shen2023difftalk} as the condition to control the model in generating the desired results. Notably, compared to GAN, the diffusion model does not require the discriminator network, thus alleviating common problems such as unstable training and mode collapse in GAN.

%Inspired  by the diffusion model \cite{ho2020denoising, rombach2022high, ho2022classifier}, it can serve as a unifying framework for generative tasks, utilizing class labels \cite{dhariwal2021diffusion}, text prompts \cite{gu2022vector}, images  \cite{chen2023diffusiondet}, and even sounds \cite{shen2023difftalk} as the condition to control the model in generating the desired results. 



%It consists of two primary stages: a forward diffusion stage that gradually adds Gaussian noise to ground truth saliency maps to obtain \textit{noisy} maps, and a reverse denoising stage that utilizes the proposed Saliency-UNet to generate the original saliency maps from the noisy input progressively.  By employing  a \textit{simple} mean square error loss as the training objective, our DiffSal is enabled to predict ground truth maps from random noisy maps.


In this paper, we present a conditional \textbf{Diff}usion framework for generalized audio-visual \textbf{Sal}iency prediction (DiffSal), which aims to tackle these two challenges simultaneously,  as illustrated in Figure \ref{fig-three-methods}(c). Our DiffSal reformulates the prediction problem as a conditional generative task of the saliency map, utilizing input video and audio as the condition.
By constructing a latent space to explore pairs of audio and visual features with spatio-temporal coherence, the obtained similar pixel-wise multi-modal features can ensure effective audio-visual interaction.
In addition, a novel Saliency-UNet is introduced to learn robust multi-modal representations across multiple scales by inductively exploiting information from both noisy maps and spatio-temporal audio-visual features.
The entire DiffSal framework employs a \textit{simple} mean square error loss as the training objective, offering a generalized approach to saliency prediction.


%By employing  a \textit{simple} mean square error loss as the training objective, our DiffSal is enabled to predict ground truth maps from random noisy maps.

%We introduce a novel Saliency-UNet with the multi-modal attention modulation desgin, enabling our model to better utilize spatio-temporal audio-visual information across multiple scales. These multi-scale visual and audio features are produced by our spatio-temproal video and audio encoders, which perform  spatial and temporal feature extraction in image sequences and corresponding audio signals. 
%In addition, the multi-modal attention modulation in Saliency-UNet facilitates learning robust multi-modal representations by inductively exploiting information from both noisy saliency maps and spatio-temporal audio-visual features. Subsquently, we use successive multi-modal attention operations across multiple scales to progressively incorporate multi-modal features until generating high-resolution results.
%To our best knowledge, we are the first to inverstigate audio-visual saliency prediction from the lens of diffusion-based generative modeling. 
%Extensive experiments demonstrate that our method greatly outperforms previous state-of-the-arts on six audi-visual saliency benchmarks.

%Unlike the vanilla diffusion model, which simply uses UNet for denoising, we propose two novel designs that enhance the capabilities of the Saliency-UNet. These modifications enable the Saliency-UNet to better utilize spatio-temporal information and generate the salient regions. We design the spatio-temporal video and audio encoders, which simultaneously perform spatial and temporal information extraction in video sequences and corresponding audio signals. The resulting audio and visual features, which contain rich spatio-temporal priors, are subsquently utilized as a fixed condition at each denoising step by the Saliency-UNet. 
%In addition, we propose multi-modal attention block in Saliency-UNet Decoder, which helps the Saliency-UNet to learn intricate representations for saliency prediction by inductively leveraging information from both noisy saliency maps and spatio-temporal audio-visual features. To be specific, we first perform elaborate multi-model feature interaction for the niosy, audio, and visual features to obtain a robust multi-modal representation. We then use efficient cross-attention operations across multiple scales to progressively incorporate multi-modal features until generating high-resolution results.


To summarize, our main contributions are:
(1) We formulate the saliency prediction problem as a conditional generative task and propose a novel conditional diffusion saliency model with the benefits of generalized network structure and effective audio-visual interaction.
(2) We design a Saliency-UNet, that can effectively incorporate audio and visual features across multiple scales to enhance performance.
(3) We condcut extensive experiments on six challenging audio-visual benchmarks. These results demonstrate that the proposed DiffSal achieves excellent performance, exhibiting an average relative improvement of 6.3\% over the previous state-of-the-art results across four metrics.


==> sec/sec_method_new.tex <==
\section{Preliminaries}
\label{sec:pre}

\begin{figure*}[!htbp]
	\centering
	\includegraphics[width=\textwidth]{figures/fig_model_structure.pdf}
%	\vspace{-10pt}
	\caption{An overview of the proposed DiffSal framework: the spatio-temporal video features $f_v$ and audio features $f_a$ are firstly encoded by the Video and Audio Encoders, respectively. Then the Saliency-UNet takes audio features $f_a$ and video features $f_v$ as the condition to guide the network in saliency map $\hat{x}_0$ generation from the noisy map $x_t$.
	}
	\label{fig-model_structure}
%	\vspace{-10pt}
\end{figure*}

Diffusion models \cite{ho2020denoising} are likelihood-based models for points sampling from a given distribution by gradually denoising random Gaussian noise in $T$ steps. In the forward diffusion process, the increased noises are added to a sample point $x_0$ iteratively as $x_0 \to \cdots \to x_{T-1} \to x_{T}$, to obtain a completely noisy image $x_T$. Formally, the forward diffusion process is a Markovian noising process defined by a list of noise scales $\{ \bar{a}_t\}^T_{t=1}$ as:
		

\begin{equation}
	\begin{aligned}
	&q(x_t|x_0) := \mathcal{N}(x_t | \sqrt{\bar{\alpha}_t}x_0, (1-\bar{\alpha}_t)\textit{\textbf{I}}), \\
	&x_t = \sqrt{\bar{\alpha}_t}x_0 + \sqrt{1-\bar{\alpha}_t}\epsilon, \epsilon \in \mathcal{N}(0, \textit{\textbf{I}}),
	\label{eq:diff_1}
	\end{aligned}
\end{equation}


\noindent where $ \bar{\alpha}_t := \prod_{s=1}^t \alpha_t = \prod_{s=1}^t (1-\beta_s)$ and $\beta_s$ denote the noise variance schedule \cite{ho2020denoising}, $\epsilon$ is the noise, $\mathcal{N}$ denotes normal distribution, $x_0$ is the original image, and $x_t$ is the generated noisy image after $t$ steps of the diffusion process.

The reverse diffusion process aims to learn the posterior distribution $p(x_{t-1} | x_0, x_t)$ for $x_{t-1}$ estimation given $x_t$. Typically, this can be done using a step-dependent neural network in multiple parameterized ways. Instead of directly predicting the noise $\epsilon$, we choose to parameterize the neural network $f_\theta(x_t, t)$ to predict $x_0$ as \cite{chen2023diffusiondet}. For model optimization, a mean squared error loss is employed to match $f_\theta(x_t, t)$ and $x_0$:

\begin{equation}
	\mathcal{L} = \| f_\theta(x_t, t) - x_0 \|^2, t \in_R {1,2, \dots, T}
	\label{eq:diff_2}
\end{equation}

\noindent where the step $t$ is randomly selected at each training iteration.
From starting with a pure noise $x_t \in \mathcal{N}(0, \textit{\textbf{I}})$ during inference stage, the model can gradually reduce the noise according to the update rule \cite{song2020denoising} using the trained $f_\theta$ as below:

\begin{equation}
	\begin{aligned}
	x_{t-1} = 	&\sqrt{\bar{\alpha}_{t-1}}f_\theta(x_t, t) +  \\
				&\sqrt{1-\bar{\alpha}_{t-1} - \sigma_s^2}\frac{x_t - \sqrt{\bar{\alpha}_t}f_\theta(x_t, t)}{\sqrt{1-\bar{\alpha}_t}} + \sigma_s \epsilon. \\
	\end{aligned}
	\label{eq:diff_3}
\end{equation}

Iteratively applying Eq. \ref{eq:diff_3}, a new sample $x_0$ can be generated from $p_\theta$ via a trajectory $x_T\to x_{T-1} \to \cdots \to x_0$. Specially, some improved sampling strategy skips such an operation in the trajectory to achieve better efficiency \cite{song2020denoising}.

To control the generation process, the conditional information can be modeled and incorporated in the diffusion model as an extra input $f_\theta(x_t, t, \mathbb{C})$. The Class labels \cite{dhariwal2021diffusion}, text prompts \cite{gu2022vector}, and audio guidance \cite{ao2023gesturediffuclip} are the prevalent forms of conditional information documented in the literature.

%Conditional information can be incorporated in the diffusion model to control the generation process. The conditional model can be represented  as $f_\theta(x_t, t, \mathbb{C})$ as an extra input. Class labels \cite{dhariwal2021diffusion}, text prompts \cite{gu2022vector}, and audio guidance \cite{ao2023gesturediffuclip} are the prevalent forms of conditional information documented in the literature.


\section{Method}
%To tackle the challenges of effective audio-visual interaction and generalized saliency network, we formulate audio-visual saliency prediction as a conditional generation task of the saliency map, utilizing input video and audio as the condition, and term the proposed method as DiffSal.  An overview of the DiffSal is illustrated in Figure \ref{fig-model_structure}.  The whole model can be divided  into two parts: the Video and Audio Encoders, as well as the Saliency-UNet.
%The Video and Audio Encoders is used to extract multi-scale spatio-temporal video features and audio features  from image sequences and corresponding audio signals.
%By conditioning on these semantic video and audio features, the Saliency-UNet performs multi-modal attention modulation to progressively refine the ground-truth saliency map from the noisy map.
%Each part is elaborated in below.

To tackle the challenges of effective audio-visual interaction and saliency network generalization, we formulate audio-visual saliency prediction as a conditional generation modeling of the saliency map, which treats the input video and audio as the condition. Figure \ref{fig-model_structure} illustrates the overview of the proposed `DiffSal', which contains parts of Video/Audio Encoders and the model of Saliency-UNet.

As shown in Figure \ref{fig-model_structure}, the Video/Audio Encoders are used to extract multi-scale spatio-temporal video features and audio features  from image sequences and corresponding audio signals. By conditioning on these semantic video and audio features, the Saliency-UNet performs multi-modal attention modulation to progressively refine the ground-truth saliency map from the noisy map. Each part of DiffSal is elaborated in below.

%Given the input video data $V \in  \mathbb{R}^{   T_v \times H_v  \times W_v \times  3 }$ and audio data $A \in \mathbb{R}^{   T_a \times H_a  \times W_a \times  1 }$,  we model audio-visual global correlations as conditions and approximate the data distribution of the ground truth saliency maps $H_0 \in \{0,1\}^{H_v \times W_v \times 1}$ based on these conditions .  The proposed DiffSal is composed of: a two-stream network to obtain visual saliency and auditory saliency feature, an audio-visual interaction module to integrate the visual and auditory conspicuity maps, a consistency-aware predictive coding module to reason the coherent spatio-temporal visual feature with audio feature, and a saliency decoder to estimate saliency map with multi-scale audio-visual features.


\subsection{Video and Audio Encoders}
\label{sec:av_encoders}

\textbf{Video Encoder}. Let $I = [I_1, \cdots, I_i, \cdots, I_{T_v}], I_i \in  \mathbb{R}^{H_v  \times W_v \times  3 }$ denotes an RGB video clip of length $T_v$.  $I$ serves as the input to a video backbone network to generate spatio-temporal feature maps. The backbone consists of 4 encoder stages and outputs 4 hierarchical video feature maps as shown in Figure \ref{fig-model_structure}. The generated feature maps are denoted as $\{\textbf{f}_{v}^{i} \}_{i=1}^{N}  \in \mathbb{R}^{ T^i_v \times h^i_v  \times w^i_v \times C_v^i} $, where $(h_v^i, w_v^i) = (H_v, W_v)/2^{i+1}, N=4$. In practical implementation, we employ the off-the-shelf MViTv2 \cite{li2022mvitv2} as a video encoder to encode the spatial and temporal information of image sequences. More generally, MViTv2 can also be replaced with other general-purpose encoders, \eg, S3D\cite{xie2018rethinking}, Video Swin Transformer\cite{liu2022video}.


% by first transforming the raw audio into a log-mel spectrogram via STFT, and then partitioning it into  $T_a$ slices of dimension $H_a \times W_a \times 1$  with the hop-window size of 11 ms.
\noindent \textbf{Audio Encoder}. To temporally synchronize the audio features with the video features in a better way, initially, we transform the raw audio into a log-mel spectrogram through Short-Time Fourier Transform (STFT). Then, the spectrogram is partitioned into $T_a$ slices of dimension $H_a \times W_a \times 1$ with a hop-window size of 11 ms.

To extract per-frame audio feature $\bar{\textbf{f}}_{a, i}$ where $i \in \{1, \cdots, T_a\}$, a pre-trained 2D fully convolutional VGGish network \cite{hershey2017cnn} is performed on AudioSet, resulting in a feature map of size $\mathbb{R}^{h_a \times w_a \times C_a}$. To improve the inter-frame consistency, we further introduce a learnable temporal enhancement module consisting of a patch embedding layer as well as a transformer layer. Then,
the audio features are rearranged in the spatio-temporal dimension and fed into the patch embedding layer to obtain $\bar{\textbf{f}}_{a} \in \mathbb{R}^{T_a \times h_a \times w_a \times C_a}$. For the retaining of temporal position information, a learnable positional embedding $\mathrm{\textbf{e}}^{pos}$ is incorporated along the temporal dimension:

\begin{equation}
	\begin{aligned}
%		& \bar{f}_a = \mathrm{VGGish(A)}, \\
%		& \bar{f}_a = \mathrm{PatchEmbed}(\bar{f}_a) + \mathrm{E_{POS}}, \\
%		& f_a = \mathrm{TransEncoder}(\bar{f}_a), \\
%		& \bar{f}_a = \mathrm{PatchEmbed}(\bar{f}_a)  \\
		&  \bar{\textbf{f}}_a = [\bar{\textbf{f}}_{a,0} + \mathrm{\textbf{e}}^{pos}_0, \cdots, \bar{\textbf{f}}_{a,{T_a}} + \mathrm{\textbf{e}}^{pos}_{T_a}],
%		& f_a = \mathrm{TransEncoder}(\bar{f}_a), \\
	\end{aligned}
\end{equation}

\noindent where $[\cdot; \cdot]$ represents concatenation operation. The processed feature is finally fed into the Multi-head Self Attention (MSA), the layer normalization (LN) \cite{ba2016layer} and the MLP layer to produce the spatio-temporal audio feature $\textbf{f}_a \in \mathbb{R}^{T_a \times h_a \times w_a \times C_a}$:

\begin{equation}
	\begin{aligned}
		%		& \bar{f}_a = \mathrm{VGGish(A)}, \\
		%		& \bar{f}_a = \mathrm{PatchEmbed}(\bar{f}_a) + \mathrm{E_{POS}}, \\
		%		& f_a = \mathrm{TransEncoder}(\bar{f}_a), \\
		%		& \bar{f}_a = \mathrm{PatchEmbed}(\bar{f}_a)  \\
%		& \bar{f}_a = [\bar{f}_{a,0} + \mathrm{\textbf{e}}^{pos}_0, \cdots, \bar{f}_{a,{T_a}} + \mathrm{\textbf{e}}^{pos}_{T_a}] \\
		& \bar{\textbf{f}}_a = \mathtt{MSA(LN(}\bar{\textbf{f}}_a)) + \bar{\textbf{f}}_a, \\
		& \textbf{f}_a = \mathtt{MLP(LN(}\bar{\textbf{f}}_a)) + \bar{\textbf{f}}_a.
%		& f_a = \mathrm{TransEncoder}(\bar{f}_a),
	\end{aligned}
\end{equation}

\subsection{Saliency-UNet}
\label{sec:sal_decoder}

Building upon the denoising process outlined in Section \ref{sec:pre}, we design a novel conditional denoising network $g_\psi$ with multi-modal attention modulation, named Saliency-UNet.
This network is designed to leverage both audio feature $\textbf{f}_a$ and video feature $\textbf{f}_v$ as the condition, guiding the model in generating the saliency map $\hat{x}_0$ from the noisy map $x_t$.

% which can take audio feature $f_a$  and video feature $f_v$ as conditions to guide the network in generating the saliency map $x_0$ from the noisy map $x_t$.

\begin{equation}
	\begin{aligned}
		& \hat{x}_0 = g_\psi(x_t, t, \textbf{f}_a, \textbf{f}_v),
	\end{aligned}
\end{equation}

The proposed Saliency-UNet can be functionally divided into two parts: feature encoding and feature decoding, as shown in Figure \ref{fig-model_structure}. The first part encodes multi-scale noisy feature maps $\{\textbf{f}_{x}^{i}\}_{i=1}^{N} \in \mathbb{R}^{h_v^i \times w_v^i \times C_v^i}$ from the noisy map $x_t$ using multiple ResNet stages. The second part utilizes our designed multi-modal attention modulation (MAM) across multiple scales for the interaction of noisy features, audio features, and video features.

The MAM stage comprises an upsampling layer, a multi-modal attention block, and a 3D temporal convolution. This stage not only computes the global spatio-temporal correlation between multi-modal features but also progressively enhances the spatial resolution of the feature maps. At last, a prediction head is employed to produce the predicted saliency map $\hat{x}_0$. The entire network contains 4 layers of the ResNet stage for feature encoding and 4 layers of the MAM stage for feature decoding.

%The MAM structure not only enables interactions between multi-modal features, but also computes global spatio-temporal correlations between audio and visual features
%Our Saliency-UNet is structurally similar to the original diffusion model \cite{ho2020denoising}, as shown in Figure \ref{fig-model_structure}, the difference being that our network replaces the standard ResNet stages in the decoder part with the designed multi-modal attention modulation stages. This choice of structure facilitates the computation of global spatio-temporal correlations between audio and visual features, while also enabling interaction between multi-modal features. The decoder part of the  Saliency-UNet network employs four multi-modal attention modulation stages, each of which consists of an upsampling operation, a multi-modal attention block, and a temporal convolution operation, respectively.
% the Saliency-UNet encoder extracts multi-scale noisy features $\{f_{x}^{i}\} (i=1, \dots, 4)$ from the noisy map $x_t$. They are then fed into the Saliency-UNet decoder along with the acquired multi-scale visual features $\{f_{v}^{i} \}(i=1, \dots, 4)$ and audio features $f_a$.  During the decoding process, we gradually incorporate interacted multimodal features and progressively reconstruct the resolution of the features until generating the saliency map.

For more robust multi-modal feature generation, two techniques in MAM are introduced: efficient cross-attention mechanism and multi-modal interaction module.

%In order to obtain robust multi-modal features, we introduce two techniques in MAM:  efficient cross-attention mechnaism and multi-modal interaction module.

% we first project the step index $t$ into an embedding and perform the multi-scale feature extraction on the initial noisy saliency map $x_t$, while incorporating step embedding in the noisy features at each scale to obtain multi-scale step-adaptive noisy features $\{f_{x}^{i}\}  \in \mathbb{R}^{ h_i  \times w_i \times C_i} (i=1, \dots, 4)$.
%Then, we model the global correlations between audio, video and noisy features across multiple scales via the well-designed decoder structures and obtain multi-scale representations. Finally, these features are integrated and passed to a prediction head to predict the saliency map $\hat{Y}_t$.


%After obtaining the  multi-scale spatio-temporal features $\{f_{v}^{i} \}(i=1, \dots, 4)$ and audio feature $f_a$, the Saliency-UNet denoises the saliency map $x_t$ by taking $\{ f_{v}^{i} \}(i=1, \dots, 4)$ and $f_a$ together with the sampling step $t$ as conditions, and output the predicted saliency map $\hat{x}_0 = \hat{Y}_t$.  Specifically, we first project the step index $t$ into an embedding and perform the multi-scale feature extraction on the initial noisy saliency map $x_t$, while incorporating step embedding in the noisy features at each scale to obtain multi-scale step-adaptive noisy features $\{f_{x}^{i}\}  \in \mathbb{R}^{ h_i  \times w_i \times C_i} (i=1, \dots, 4)$.  Then, we model the global correlations between audio, video and noisy features across multiple scales via the well-designed decoder structures and obtain multi-scale representations. Finally, these features are integrated and passed to a prediction head to predict the saliency map $\hat{Y}_t$.

\noindent \textbf{Efficient Cross-Attention Mechanism}. Given video feature $\textbf{f}_{v}^{i} \in \mathbb{R}^{T_v^i \times h_v^i \times w_v^i \times C_v^i }$, audio feature $\textbf{f}_a \in \mathbb{R}^{T_a \times h_a \times w_a \times C_a}$ and noisy feature $\textbf{f}_{x}^{i} \in \mathbb{R}^{h_v^i \times w_v^i \times C_v^i}$, the video feature and noisy feature are concatenated as a spatio-temporal noisy feature $[\textbf{f}_{v}^i; \textbf{f}_{x}^i]\in \mathbb{R}^{(T_v^i +1) \times h_v^i \times w_v^i \times C_v^i }$. The processed feature is then fed into the multi-modal interaction module along with the audio feature to obtain $\textbf{f}_{avx} \in \mathbb{R}^{(T_v^i +1) \times h_v^i \times w_v^i \times C_v^i }$.

When all the processed features have been obtained, we find that it would take a prohibitively large amount of memory due to the high spatio-temporal resolution of the feature map, if directly following the standard cross-attention \cite{rombach2022high}.

%After acquiring all the processed features, we find that directly  following the standard cross-attention \cite{rombach2022high} would take a prohibitively large amount of memory due to the high spatio-temporal resolution of the feature map.


Inspired by spatial-reduction attention in PVT \cite{wang2021pyramid}, a spatio-temporal reduction operation is further applied to key ${K}$ and value ${V}$, which drastically reduces the computation and memory overhead as below:


\begin{equation}
	\begin{aligned}
		{Q} &= {V} = [\textbf{f}_{v}^i; \textbf{f}_{x}^i]; {K} = \textbf{f}_{avx}^i, \\
		\textbf{f}_{avx}^i &= \mathtt{Attn}( Q W_Q, \mathtt{STR}(K)W_K, \mathtt{STR}(V)W_V), \\
	\end{aligned}
\end{equation}

\noindent where $W_Q, W_K, W_V \in \mathbb{R}^{C_i \times C_i} $ are parameters of linear projections, $\mathtt{STR(\cdot)}$ is the spatio-temporal reduction, which is defined as:

\begin{equation}
	\begin{aligned}
		& \mathtt{STR}(x) = \mathtt{LN(Conv3d}(x)),
	\end{aligned}
\end{equation}

\noindent Here, the dimension of features is reduced by controlling the kernel size as well as the stride size of 3D convolution.

\noindent \textbf{Multi-modal Interaction Module}. To take full advantage of different modal features, the interaction is modeled between audio feature $\textbf{f}_a$, video feature $\textbf{f}_v^{i}$ and noisy feature $\textbf{f}_{x}^i$ at each scale $i$ to obtain a robust multi-modal feature representation. A straightforward method is to directly concatenate and aggregate $\textbf{f}_a$, $\textbf{f}_v^{i}$ and $\textbf{f}_{x}^i$, but such a simple fusion does not acquire global correlations between various modalities. Therefore, an effective multi-modal interaction strategy is proposed to capture crucial audio-visual activity changes in the spatio-temporal domain. In specific, this process starts with convolution and upsampling on the audio feature, which is to construct spatially size-matched feature triples $(\widetilde{\textbf{f}}_a, \textbf{f}_v^i, \textbf{f}_x^i)$.

Subsequently, the video feature and noisy feature are concatenated to obtain spatio-temporal noisy features $[\textbf{f}_{v}^i; \textbf{f}_{x}^i]$. The processed feature undergoes an element-wise product operation with the audio feature, and outputs $\bar{\textbf{f}}_{avx}^i$. We then perform average activation along the temporal dimension over $\bar{\textbf{f}}_{avx}^i$ to pool global temporal information into a temporal descriptor. For the indication of critical motion regions, a softmax function is applied to obtain a mask by highlighting the segments of the corresponding spatio-temporal audio features, which exhibits key audio-visual activity changes.

%The video feature and noisy feature are then concatenated together to obtain spatio-temporal noisy features $[f_{v}^i; f_{x}^i]$. This processed feature is subjected to an element-wise product operation with the audio feature to yield $\bar{f}_{avx}^i$. Subsequently, we take the average activation along the temporal dimension over $\bar{f}_{avx}^i$ to pool the global temporal information into a temporal descriptor, followed by a softmax function to obtain a mask that indicates the critical motion region. Finally, the mask is utilized to highlight segments of the corresponding spatio-temporal noise features that have key audio-visual activity changes.

\begin{equation}
	\begin{aligned}
		 \widetilde{\textbf{f}}_a &= \mathtt{Conv}(\mathtt{UpSample}(\textbf{f}_a)),\\
		\textbf{f}_{avx}^i &= \mathtt{softmax}(\mathtt{Pool}([\textbf{f}_{v}^i; \textbf{f}_{x}^i] \ast \widetilde{\textbf{f}}_a)) \ast \widetilde{\textbf{f}}_a.  \\
	\end{aligned}
\end{equation}

\noindent where $\mathtt{Conv}(\cdot)$,  $\ast$, $\mathtt{softmax}$ and $\mathtt{Pool}$ denote the operations of convolution, element-wise product, softmax and average pooling, respectively.

%\noindent \textbf{Saliency Map Generation}.
%Finally, we employ a prediction head to yield the predicted saliency map $\hat{Y}_t$.
%
%Ultimately, we integrate feature representations across all scales $\{\mathcal{F}_1,  \mathcal{F}_2, \mathcal{F}_3, \mathcal{F}_4 \}$ via element-wise addition, and employ a prediction head to yield the predicted saliency map $\hat{Y}_t$. By inductively modeling multi-scale feature interactions, our Saliency-UNet is able to reason about the fine-grained relationships between key saliency regions and global contexts, thereby producing more tailored representations that attend to joint audio-visual activity.
%


\subsection{Overall Training and Inference}
\label{sec:training}

%\textbf{Training}. We initiate a diffusion process that introduces corruption to ground-truth saliency maps, creating noisy maps. Subsequently, we train the Saliency-UNet for saliency map denoising, aiming to reverse this process. The overall training procedure of our DiffSal is outlined in Algorithm \ref{alg:training} in the Appendix. In detail, we sample Gaussian noises following $\alpha_t$ in Eq. \ref{eq:diff_1} and add them to ground-truth saliency maps, resulting in noisy samples. The parameter $\alpha_t$ at each sampling step $t$ is pre-defined by a monotonically decreasing cosine scheme, as employed in \cite{ho2020denoising}. The standard mean square error serves as the optimization function to supervise the model training:
%\begin{equation}
%	\begin{aligned}
%		& \mathcal{L} =  \| x_0 - g_\psi(x_t, t, \textbf{f}_a, \textbf{f}_v) \|^2. \\
%	\end{aligned}
%\end{equation}
%
%\noindent where $x_0$ and $g_\psi(x_t, t, \textbf{f}_a, \textbf{f}_v)$ denote the ground-truth and predicted saliency maps, respectively.
%
%
%\noindent \textbf{Inference}. The proposed DiffSal engages in denoising on noisy saliency maps sampled from a Gaussian distribution, progressively refining its predictions across multiple sampling steps. In each sampling step, the Saliency-UNet processes random noisy saliency maps or the predicted saliency maps from the previous sampling step as input, producing estimated saliency maps for the current step. Subsequently, we apply DDIM \cite{song2020denoising} to update the saliency maps for the next step. The detailed inference procedure is outlined in Algorithm \ref{alg:infer}.

\textbf{Training}. A diffusion process is initiated to create noisy maps by introducing corruption to ground-truth saliency maps. To reverse this process, the Saliency-UNet is trained for saliency map denoising. The overall training procedure of DiffSal is outlined in Algorithm \ref{alg:training} in the Appendix. In detail, Gaussian noises are sampled following $\alpha_t$ in Eq. \ref{eq:diff_1} and added to the ground-truth saliency maps, resulting in noisy samples. At each sampling step $t$, the parameter $\alpha_t$ is pre-defined by a monotonically decreasing cosine scheme, as employed in \cite{ho2020denoising}. The standard mean square error serves as the optimization function to supervise the model training.

\begin{equation}
	\begin{aligned}
		& \mathcal{L} =  \| S_0 - g_\psi(S_t, t, \textbf{f}_a, \textbf{f}_v) \|^2.
	\end{aligned}
\end{equation}

\noindent where $S_0$ and $g_\psi(S_t, t, \textbf{f}_a, \textbf{f}_v)$ denote the ground-truth and predicted saliency maps, respectively.


\noindent \textbf{Inference}. The proposed DiffSal engages in denoising on noisy saliency maps sampled from a Gaussian distribution, and progressively refines the corresponding predictions across multiple sampling steps. In each sampling step, the Saliency-UNet processes random noisy saliency maps or the predicted saliency maps from the previous sampling step as input, and generates the estimated saliency maps for the current step. For the next step, DDIM \cite{song2020denoising} is applied to update the saliency maps. The detailed inference procedure is outlined in Algorithm \ref{alg:infer}. 

==> sec/sec_related.tex <==
\section{Related Work}
\label{sec:related}


%\subsection{Video Saliency Prediction}
%For video saliency prediction, different strategies of modeling temporal motion information have been proposed to estimate the saliency maps over consecutive frames \cite{bak2018spatio, min2019tased, jain2021vinet}. Bak \etal \cite{bak2018spatio} propose a two-stream spatio-temporal network to process video frames with optical flow maps, simultaneously. The Long-Short Term Memory (LSTM) \cite{hochreiter1997long}  and Gated Recurrent Unit (GRU) \cite{chung2014empirical} have also been incorporated into the video saliency prediction, and subsequently Wang \etal \cite{wang2018revisiting} propose to combine the Conv-LSTM with dynamic attention mechanism into a network to further enhance the prediction performance. Similarly to model long-term temporal characteristics, Lai \etal \cite{lai2019video} propose STRA-Net based on a lightweight convGRU. After Min \etal \cite{min2019tased} adopt a S3D model \cite{xie2018rethinking} to build TASED-Net with 3D convolutions, the training paradigm of 3D convolution has been widely used in the VSP task. Bellitto \etal \cite{bellitto2020video} design a 3D fully convolutional architecture to obtain multi-scale saliency instances for the combination of output saliency maps. Jain \etal  \cite{jain2021vinet}  adopt a 3D encoder-decoder structure in a U-Net-like fashion, this enables the decoding features of various layers to be constantly concatenated with the corresponding feature of an encoder in the temporal dimension. Also benefit from spatio-temporal modeling of 3D convolution but unlike previous works, a novel saliency decoder is designed in our work to perform aggregation of the multi-scale features.


\subsection{Audio-Visual Saliency Prediction}
For audio-visual saliency prediction, different strategies of modeling multi-modal correlations have been proposed to estimate the saliency maps over consecutive frames.
Early approaches \cite{min2016fixation, min2020multimodal} attempted to localize the moving-sounding target by using canonical correlation analysis (CCA) to establish the cross-modal connections between the two modalities.
With the advent of deep learning, Tsiami et al. \cite{tsiami2020stavis} continued the localization-based approach by extracting audio representation using SoundNet \cite{aytar2016soundnet} and performing spatial sound source localization through bilinear operation \cite{tenenbaum2000separating}. 
However, these methods exhibited sub-optimal performance, leading to the emergence of more effective 3D convolution-based approaches \cite{tavakoli2019dave, jain2021vinet, xiong2023casp} that employ encoder-decoder architectures.
For example, Jain \etal \cite{jain2021vinet} and Xiong \etal \cite{xiong2023casp} both embrace the UNet-style encoder-decoder structure, incorporating their empirical designs into the decoder. In addition, Chang \etal \cite{chang2021temporal} employs a complex hierarchical feature pyramid network to aggregate deep semantic features. 
Both the localization-based and 3D convolution-based methods use tailored network structures and sophisticated loss functions to predict saliency areas.
In contrast, we formulate the saliency prediction problem as a conditional generation task and propose a novel conditional diffusion model for generalized audio-visual saliency prediction.



%Early audio-visual saliency prediction methods attempted to establish the cross-modal connections between the two modalities by using CCA ,but an end-to-end deep learning scheme is still far from in-depth study. More recently, Tavakoli \etal \cite{tavakoli2019dave} propose to train two independent 3D ResNet for audio and visual modalities, and the outputs are directly concatenated as a late fusion strategy. With SoundNet \cite{aytar2016soundnet} for audio representation learning, Tsiami \etal\cite{tsiami2020stavis} perform a spatial sound source localization to obtain audio features, which are then fused with the visual feature maps by bilinear operation. In the same way, Jain \etal \cite{jain2021vinet} also employ bilinear fusion operation on the audio features of SoundNet and visual features to predict saliency maps. For these solutions based on a bilinear-based fusion scheme, the large number of learning parameters causes the model learning not easy to converge \cite{tenenbaum2000separating, yu2017multi}. In our work, an attention-based fusion is exploited to learn the cross-modal semantic interaction to overcome such a limitation.

%\subsection{Audio-Visual Learning}

\begin{figure*}[!htbp]
	\centering
	\includegraphics[width= \textwidth]{figures/fig_model_structure.pdf}
	\vspace{-15pt}
	\caption{An overview of the proposed DiffSal framework. DiffSal first encodes  spatio-temporal video features $\textbf{f}_v$ and audio features $\textbf{f}_a$ by the Video and Audio Encoders, respectively.
		Then the Saliency-UNet takes audio features $\textbf{f}_a$  and video features $\textbf{f}_v$ as the condition to guide the network in generating the saliency map $\hat{S}_0$ from the noisy map $S_t$.
	}
	\label{fig-model_structure}
	\vspace{-10pt}
\end{figure*}

\subsection{Diffusion Model}
In recent years, diffusion models have gained significant traction in the field of deep learning. During the diffusion process, they employ Markov processes to introduce noise into the training data and then train deep neural networks to reverse it. Thanks to the high-quality generative results and strong generalization capabilities, diffusion models have achieved significant success in generative tasks, such as image generation\cite{austin2021structured,benny2022dynamic,bond2022unleashing,choi2022perception,de2021diffusion}, image-to-image translation\cite{saharia2022palette,zhao2022egsde,wang2022pretraining,li2022vqbb,wolleb2022swiss}, video generation\cite{harvey2022flexible,yang2022diffusion,hoppe2022diffusion}, text-to-image synthesis\cite{gu2022vector,ramesh2022hierarchical,zhang2022fast}, and more. Beyond generative tasks, diffusion models have proven to be highly effective in various computer vision tasks. For instance, DiffSeg\cite{amit2021segdiff} proposes a diffusion model conditioned on an input image for image segmentation. Chen \etal \cite{chen2023diffusiondet} propose a method called DiffusionDet, which formulates object detection as a generative denoising process from noisy boxes to object boxes. Subsequently, Gu \etal \cite{gu2022diffusioninst} extend the DiffusionDet pipeline  by introducing noise filters during diffusion and incorporating a mask branch for global mask reconstruction, making it applicable to instance segmentation tasks. To the best of our knowledge, there have been no previous successful attempts to apply diffusion models to saliency prediction. The proposed DiffSal in this paper explores the potential of diffusion models in the domain of audio-visual saliency prediction.




